Rubin Science Platform on Google: the story so far

We describe Rubin Observatory's experience with offering a data access facility (and associated services including our Science Platform) deployed on Google Cloud infrastructure as part of our pre-Operations Data Preview program.

==> Makefile <==
DOCNAME = O3-2

tex = $(filter-out $(wildcard *acronyms.tex) , $(wildcard *.tex))

GITVERSION := $(shell git log -1 --date=short --pretty=%h)
GITDATE := $(shell git log -1 --date=short --pretty=%ad)
GITSTATUS := $(shell git status --porcelain)
ifneq "$(GITSTATUS)" ""
	GITDIRTY = -dirty
endif

export TEXMFHOME ?= lsst-texmf/texmf

#$(DOCNAME).pdf: $(tex) meta.tex O3-002.bib authors.tex acronyms.tex
#	latexmk -bibtex -xelatex -f $(DOCNAME)

O3-002.pdf: $(tex) $(DOCNAME).bib 
	latex $(DOCNAME)
	bibtex $(DOCNAME)
	latex $(DOCNAME)
	latex $(DOCNAME)
	dvipdfm $(DOCNAME)
	dvipdf $(DOCNAME)

# Acronym tool allows for selection of acronyms based on tags - you may want more than DM
acronyms.tex: $(tex) myacronyms.txt
	$(TEXMFHOME)/../bin/generateAcronyms.py -t "DM" $(tex)

# Remove the USA from the author list since that can be assumed
authors.tex:  authors.yaml
	python3 $(TEXMFHOME)/../bin/db2authors.py --mode adass > authors.tex
	perl -pi -e 's|, USA||' authors.tex

.PHONY: clean
clean:
	latexmk -c
	rm -f $(DOCNAME).bbl
	rm -f $(DOCNAME).out
	rm -f $(DOCNAME).dvi
	rm -f $(DOCNAME).xdv
	rm -f meta.tex

.FORCE:

meta.tex: Makefile .FORCE
	rm -f $@
	touch $@
	echo '% GENERATED FILE -- edit this in the Makefile' >>$@
	/bin/echo '\newcommand{\lsstDocType}{$(DOCTYPE)}' >>$@
	/bin/echo '\newcommand{\lsstDocNum}{$(DOCNUMBER)}' >>$@
	/bin/echo '\newcommand{\vcsRevision}{$(GITVERSION)$(GITDIRTY)}' >>$@
	/bin/echo '\newcommand{\vcsDate}{$(GITDATE)}' >>$@


==> abstract.tex <==

\begin{abstract}

We describe Rubin Observatory's experience with offering a data access facility (and associated services including our Science Platform) deployed on Google Cloud infrastructure as part of our pre-Operations Data Preview program.
\end{abstract}

==> acronyms.tex <==
\addtocounter{table}{-1}
\begin{longtable}{p{0.145\textwidth}p{0.8\textwidth}}\hline
\textbf{Acronym} & \textbf{Description}  \\\hline

CA & Control (or Cost) Account \\\hline
DC2 & Data Challenge 2 (DESC) \\\hline
DESC & Dark Energy Science Collaboration \\\hline
DMTN & DM Technical Note \\\hline
DP & Data Production \\\hline
DP0 & Data Preview 0 \\\hline
DP1 & Data Preview 1 \\\hline
DP2 & Data Preview 2 \\\hline
GCS & Generic Control System \\\hline
IDF & Interim Data Facility \\\hline
IPAC & No longer an acronym; science and data center at Caltech \\\hline
IR & infrared \\\hline
LSST & Legacy Survey of Space and Time (formerly Large Synoptic Survey Telescope) \\\hline
NCSA & National Center for Supercomputing Applications \\\hline
PB & PetaByte \\\hline
PanDA &  Production ANd Distributed Analysis system \\\hline
RSP & Rubin Science Platform \\\hline
RTN & Rubin Technical Note \\\hline
SLAC & SLAC National Accelerator Laboratory \\\hline
SQR & SQuARE document handle \\\hline
US & United States \\\hline
USDF & United States Data Facility \\\hline
\end{longtable}

